High-Level, Collaborative Task Planning Grammar and Execution for Heterogeneous Agents

We propose a new multi-agent task grammar to encode collaborative tasks for a team of heterogeneous agents that can have overlapping capabilities. The grammar allows users to specify the relationship between agents and parts of the task without providing explicit assignments or constraints on the number of agents required. We develop a method to automatically find a team of agents and synthesize correct-by-construction control with synchronization policies to satisfy the task. We demonstrate the scalability of our approach through simulation and compare our method to existing task grammars that encode multi-agent tasks.

==> Sections/Definitions.tex <==




A robot model $A_j$ is the product of its motion model and $k = |\Lambda_j|$ capabilities: $A_j = \lambda_{\mathit{Mot,j}} \times \lambda_1 \times \lambda_2 ... \times \lambda_k$ such that $A_j=(S, s_0, AP_j, \gamma, L, W)$, where 

\begin{itemize}
    \item $S = S_{\mathit{Mot,j}} \times S_1 \times S_2 \times ... \times S_k$ is the set of states
    \item $s_0 \in S$ is the initial state
    \item $AP_j = AP_{Mot,j} \cup (\bigcup_{i=1}^k AP_i)$ is the set of propositions
    \item $\gamma \subseteq S \times S$ is the transition function such that $(s,s')\in \gamma$, where $s = (s_{\mathit{Mot,j}}, s_1, s_2, ..., s_k), s' = (s'_{\mathit{Mot,j}}, s'_1, s'_2, ..., s'_k)$, if and only if $(s_{\mathit{Mot,j}}, s'_{\mathit{Mot,j}}) \in \Delta_{\mathit{Mot,j}}$  and for $i=\{1,...,k\}, (s_i, s'_i) \in \Delta_i$
    \item $L:S \rightarrow 2^{AP_j}$ is the labeling function where $L(s) = L_{Mot,j}(s_{\mathit{Mot,j}}) \cup (\bigcup_{i=1}^k L_i(s_i))$
    % \hkc{$L(s) = L_{\mathit{Mot,j}}(s_{\mathit{Mot,j}})\cup L_1(s_1)\cup L_2(s_2)\cup ... ,\cup L_k(s_k)$}
    \item $W: \gamma \rightarrow \mathbb{R}_{\ge 0}$ is the cost function. 
    
\end{itemize}

\bigskip
\noindent $\Sigma_{\mathcal{B}} = 2^{AP_{\varphi}^{\psi} \cup AP_s} \times 2^{AP_{\varphi}^{\psi} \cup AP_s}$, where for $(\sigma_T, \sigma_F) \in \Sigma_\mathcal{B}$, $\sigma_T$ is the set of propositions that are true, and $\sigma_F$ is the set of propositions that are false. \hkc{this needs to be connect to the buchi} \amy{to think about- do i need additional properties/restrictions?}

% \noindent $\Sigma_\mathcal{G} = 2^{AP_j \cup AP_\varphi^{\psi} \cup AP_s}$

% \noindent $\Sigma_\mathcal{G} = (\bigcup_{\sigma \in 2^{AP_\varphi}} \sigma) \cup 
% \Sigma_j$

% \noindent $\Sigma_\mathcal{G} = \{\sigma \cup 
% \Sigma_j \ | \ \sigma \in 2^{AP_\varphi} \}$
\begin{definition}[Binding Function]
$\mathfrak{B}: \Sigma_{\mathcal{B}} \rightarrow 2^{\APbinding}$ such that for $(\sigma_T, \sigma_F) \in \Sigma_{\mathcal{B}}, \mathfrak{B}((\sigma_T, \sigma_F)) \subseteq \APbinding$ is the set $\{\rho \in\APbinding \ | \ \exists \pi^\rho \in \sigma_T \cup \sigma_F \}$. Intuitively, it is the set of bindings that appear in label $\sigma$ of a \buchi transition.
\end{definition}

% \begin{definition}[Capability  Function - True]
% $\mathfrak{C}_T: \Sigma_{\mathcal{B}} \times \APbinding \rightarrow 2^{\APltl}$ such that for $(\sigma_T, \sigma_F) \in \Sigma_{\mathcal{B}}, \rho \in \APbinding,  \Rho_T((\sigma_T, \sigma_F), \rho) = \{\pi \in\APltl \ | \ \exists \pi^\rho \in \sigma_T\}$. Intuitively, $\mathfrak{C}_T$ is the set of action and motion propositions that are true and appear with binding $\rho$ in label $\sigma$ of a \buchi transition. %of $\APltl$ that needs to be satisfied by the binding $\rho$
% \end{definition}

% \begin{definition}[Capability  Function - False]
% $\mathfrak{C}_F: \Sigma_{\mathcal{B}} \times \APbinding \rightarrow 2^{\APltl}$ such that for $(\sigma_T, \sigma_F) \in \Sigma_{\mathcal{B}}, \rho \in \APbinding,  \Rho_F((\sigma_T, \sigma_F), \rho) = \{\pi \in\APltl \ | \ \exists \pi^\rho \in \sigma_F\}$. Intuitively, $\mathfrak{C}_F$ is the set of action and motion propositions that are false and appear with binding $\rho$ in label $\sigma$ of a \buchi transition. %of $\APltl$ that needs to be satisfied by the binding $\rho$
% \end{definition}

\begin{definition}[Capability  Function]
$\mathfrak{C}_F: \Sigma_{\mathcal{B}} \times \APbinding \rightarrow 2^{\APltl} \times 2^{\APltl}$ such that for $(\sigma_T, \sigma_F) \in \Sigma_{\mathcal{B}}, \rho \in \APbinding$,$  \mathfrak{C}((\sigma_T, \sigma_F), \rho) = (C_T, C_F)$, where $C_T = \{\pi \in\APltl \ | \ \exists \pi^\rho \in \sigma_T\}$ and $C_F = \{\pi \in\APltl \ | \ \exists \pi^\rho \in \sigma_F\}$. Intuitively, $C_T$ is the set of action and motion propositions that are true and appear with binding $\rho$ in label $\sigma$ of a \buchi transition. For example, for the transition $(z, \sigma, z
)$ where $z = 1, z'= 2, \pi_2^s \in \sigma_T$, $\mathfrak{C}(\sigma, 1) = (\emptyset, \{room_A\})$. %of $\APltl$ that needs to be satisfied by the binding $\rho$
\end{definition}



 

\begin{definition}[Binding Assignment Function]
Let $q = (s, z)$, $q' = (s',z')$, $(\sigma_T, \sigma_F) \in \Sigma_{\mathcal{B}}$. Then $\mathfrak{R}(q, \sigma, q') = \{r \in 2^{\APbinding} \ | \ \forall \rho \in r, (C_T, C_F)= \mathfrak{C}((\sigma_T, \sigma_F), \rho),  \bigcup_{\rho \in r} C_T \subseteq L(s')$ and $\bigcup_{\rho \in r} C_F \not \subseteq L(s') \}$.
\end{definition}

Given $A_j = (S,s_0,AP_j, \gamma,L,W)$ and $\mathcal{B}= (Z,  z_0, \Sigma_{\mathcal{B}}, \delta_{\mathcal{B}}, F)$ and using the binding assignment function $\mathfrak{R}$, we define the product automaton $\mathcal{G}_j = A_j \times \mathcal{B}$ as:

\noindent $\mathcal{G}_j = (Q, q_0, AP_j, \Sigma_\mathcal{B},\delta_\mathcal{G},L_\mathcal{G}, W_\mathcal{G}, F_\mathcal{G})$, where 

\begin{itemize}
    \item $Q = S \times Z$ is a finite set of states
    \item $q_0 = (s_0, z_0) \in Q$ is the initial state
    % \item $\Sigma_\mathcal{G} = 2^{AP_j \cup AP_\varphi^{\psi} \cup AP_s}$ is the input alphabet
    \item $\delta_\mathcal{G}\subseteq Q\times\Sigma_\mathcal{B}\times Q$ is the transition function, where a transition exists from $q = (s, z)$ to $q' = (s',z')$ if and only if $(s,s') \in \gamma$ and $\exists \sigma \in \Sigma_{\mathcal{B}}$ such that for $(z, \sigma, z') \in \delta_{\mathcal{B}}$ and $\mathfrak{R}(q, \sigma, q') \neq \emptyset$ 
    
    % \begin{itemize}
    %     \item $(s,s') \in \gamma$
    %     \item $\exists \sigma \in \Sigma_{\mathcal{G}}$ such that $D(q, \sigma, q') \neq \emptyset$, and $z' \in \delta_{\mathcal{B}}(z, \sigma, z')$ 

    % \end{itemize}
    
   
    
    % \item $\Rho_\mathcal{G}$ is the binding function such that for all $(q, \sigma, \pi_s) \in \delta$, $\Rho(\sigma)$ maps each proposition $\APltl$ in $\sigma$ to its corresponding $\APbinding$
    \item $L_\mathcal{G}$ is the labeling function such that for $q = (s, z) \in Q$, $L_\mathcal{G}(q) = L(s)\subseteq AP_j$
    \item $W_\mathcal{G}: \delta_{\mathcal{G}} \rightarrow \mathbb{R}_{\ge 0} $ is the cost function such that for $(q, \sigma, q') \in \delta_{\mathcal{G}}$, where $q = (s, z)$ and $q' = (s',z')$, $W_\mathcal{G}((q, \sigma, q'))=W((s, s'))$
    \item $F_\mathcal{G} = S \times F$ is a set of accepting states

\end{itemize}

  
 $\mathfrak{R}((s_1,1), \sigma, (s_2,2)) = 2^{\{1,2,3\}} \setminus \emptyset$ 
 
$\mathfrak{R}((s_1,1), \sigma, (s_3,2)) = \{\{2\},\{3\},\{2,3\}\}$

$\mathfrak{R}((s_1,1), \sigma,(s_4,2)) = \{\{2\}\}$

==> Sections/RelatedWork.tex <==


\pagebreak\section{Drafting}

\begin{itemize}
    \item Heterogeneous multi-robot systems consist of robots with different capabilities
    \item collaborative tasks have been of particular interest but adds increasing complexity
    \item coalition
    \item OR scheduling
    \item TL heterogeneous teams
    \item TL collaborative tasks
\end{itemize}

Sections:
\subsection{Multi robot/agent coordination or task allocation}
\begin{itemize}
    \item coalition
    \item OR scheduling
\end{itemize}

\subsection{Coordination for TL teams}
Global tasks:

\begin{itemize}
    \item homogeneous robotic swarms for universal specification
    \begin{itemize}
        \item J. Chen, R. Sun and H. Kress-Gazit, "Distributed Control of Robotic Swarms from Reactive High-Level Specifications," 2021.
        \item M. Kloetzer and C. Belta, “Temporal logic planning and control of robotic swarms by hierarchical abstractions,” 2007.
    \end{itemize}
        
    \item "tasks that do not explicitly allocate tasks to robots typically need to be decomposed in order to obtain the required allocation"
    
    \begin{itemize}
        \item P. Schillinger, M. Burger, and D. V. Dimarogonas, “Simultaneous task allocation and planning for temporal logic goals in heterogeneous multi-robot systems,” 
        \item  Faruq, F., Parker D., Laccrda B., and Hawes, N., “Simultaneous Task Allocation and Planning Under Uncertainty,”
    \end{itemize}
    
    \item "Temporal logic control synthesis without an explicit assignment of robots to tasks has been considered"
        \begin{itemize}
        \item Y. Chen, X. C. Ding, A. Stefanescu, and C. Belta,
        “Formal approach to the deployment of distributed robotic teams”
        \item  B. Lacerda and P. U. Lima, “Petri net based multi-robot task coordination from temporal logic specifications”
    \end{itemize}
    
    
\end{itemize}

The above are all approaches that do not consider cooperative tasks that require synchronization.

Synchronization:
\begin{itemize}
    \item Y. E. Sahin, P. Nilsson and N. Ozay, "Synchronous and asynchronous multi-agent coordination with cLTL+ constraints," 2017. 
    Y. E. Sahin, P. Nilsson, and N. Ozay, “Provably-correct
coordination of large collections of agents with counting
temporal logic constraints,”
    "to capture constraints on the number of robots that must be present in different regions."

    \item STyLuS\text{*}  requires global LTL specifications that explicitly assign tasks to robots.
    \item "capture constraints on the number of robots and type of robots that must be present in different regions"
    \begin{itemize}
        
        \item Jones, A.; Leahy, K.; Vasile, C.; Sadraddini, S.; Serlin, Z.; Tron, R.; and Belta, C. “ScRATCHS: Scalable and Robust Algorithms for Task-based Coordination from High-level Specifications”, 2019.
        \item Luo, Xusheng and Michael M. Zavlanos. “Temporal Logic Task Allocation in Heterogeneous Multi-Robot Systems,” 2021
        \item centralized method
        \item Ruofei Bai, Ronghao Zheng, Yang Xu, Meiqin Liu, and Senlin Zhang. “Hierarchical multi-robot strategies synthesis and optimization under individual and collaborative temporal logic specifications”, 2021.
        

    \end{itemize}
    \item A. Mosca, C.-I. Vasile, C. Belta, and D. M. Raimondo, “Multi-
robot routing and scheduling with temporal logic and synchronization
constraints,” 
\end{itemize}

